Going Beyond Linear RL: Sample Efficient Neural Function Approximation

Deep Reinforcement Learning (RL) powered by neural net approximation of the Q function has had enormous empirical success. While the theory of RL has traditionally focused on linear function approximation (or eluder dimension) approaches, little is known about nonlinear RL with neural net approximations of the Q functions. This is the focus of this work, where we study function approximation with two-layer neural networks (considering both ReLU and polynomial activation functions). Our first result is a computationally and statistically efficient algorithm in the generative model setting under completeness for two-layer neural networks. Our second result considers this setting but under only realizability of the neural net function class. Here, assuming deterministic dynamics, the sample complexity scales linearly in the algebraic dimension. In all cases, our results significantly improve upon what can be attained with linear (or eluder dimension) methods.

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
	\item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
	\answerYes{Our abstract and introduction accurately reflect our main contribution. }
	\item Did you describe the limitations of your work?
	\answerYes{In the Preliminary section we clearly state the settings we considered and when our results apply. }
	\item Did you discuss any potential negative societal impacts of your work?
	\answerNo{Our work is theoretical and generally will not have negative social impacts.}
	\item Have you read the ethics review guidelines and ensured that your paper conforms to them?
	\answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
	\item Did you state the full set of assumptions of all theoretical results?
	\answerYes{The assumptions are clearly included in every theorem or lemma. }
	\item Did you include complete proofs of all theoretical results?
	\answerYes{All the proofs can be found in the appendix}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNA{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
    \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
    \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/poly.tex.Kaixuan.back.tex <==

\subsection{Deterministic Transitions and Generative Model}

%Setting: we obtain $N$ samples from each state-action pair. 
%
%Assumption: for every $h = 1, \cdots, H$, the set $\{\phi_h(s, a) \mid s \in \gS, a \in \gA\}$ is generic.
%\jnote{Jiaqi: State algorithm?} \jnote{All proofs go in supplementary, deadline is 6-4 for proofs.} \jnote{State setting! what's the assumption on Q*????}

\begin{definition}[Admissible Polynomial Family]
Define $\mathcal{X}: = \left\{\begin{bmatrix} 1 \\ x \end{bmatrix}^{\otimes p}: x \in \mathbb{R}^d\right\}$. Define $\F_{\gV}:=\{f_\Theta(x)= \left\langle \Theta, \begin{bmatrix} 1 \\ x \end{bmatrix}^{\otimes p}\right \rangle: \Theta \in \mathcal{V}  \}$ for a variety $\mathcal{V}$ as a polynomial family. $\F_{\gV}$ is said to be admissible\footnote{Admissible means the dimension of $\mathcal{X}$ decreases by one when there is an additional linear constraint $\langle \Theta, X\rangle =0$} wrt $\mathcal{X}$ if for any $\Theta \in \gV$, $\text{dim}(\mathcal{X} \cap \{X \in \mathcal{X} : \langle X,  \Theta\rangle =0\rangle\}  )< \text{dim}(\mathcal{X})=d $. 
%The dimension $D$ of the family is the algebraic dimension of the variety $\mathcal{V}$. 

The dimension $D$ of the family is the dimension of $\gV$.

%We further assume that $\mathcal{V}$ is the finite union of irreducible algebraic varieties\footnote{This can be weakened to containment in the finite union of irreducible varieties.}.

\end{definition}
\begin{theorem}[\cite{Anonymous}]
%	\textcolor{red}{\bf JIAQI Please summarize the bandit theorem here that we invoke}
%	
%	Let $\mathcal{V}$ be the finite union of irreducible algebraic varieties and the Minkowski set difference $\mathcal{V} - \mathcal{V}$ has  dimension $D$. Consider a polynomial family  $p_\Theta(x)= \left\langle \Theta, \begin{bmatrix} 1 \\ x \end{bmatrix}^{\otimes p}\right \rangle$ with coefficients $\Theta \in \mathcal{V}$.
% Then for any $n\ge D$, there is a unique solution (or no solution) $\Theta^\ast$ to the system of equations $y_i = p_\Theta(x_i)$, for almost all $(x_1,\ldots, x_n)$ with respect to the product measure on $\mathbb{R}^{d} \times \cdots \times \mathbb{R}^d$.
Consider the polynomial family $\F_{\gV}$ of dimension $D$.  For $n \ge 2D$, there is a unique solution (or no solution) to the system of equations $y_i =f(x_i)$ for $f \in \F_{\gV}$ almost surely with respect to the product measure on $\mathbb{R}^d \times \ldots \mathbb{R}^d$.



	\end{theorem}
\begin{assumption}[Polynomial Realizability]
For all $ h \in [H]$,  $Q^\ast_h \in \F_{\gV}$ for an admissible polynomial family.
\end{assumption}

%\jnote{What is r???} what's the model class???? ??? 
\begin{theorem} Assume that the set $\{\phi_h(s,a) \mid s\in \gS, a \in \gA \}$ is generic at any level $h$. Under the polynomial realizability, Algorithm \ref{alg:querypoly} learns the optimal policy $\pi^\star$ with at most  $N = 2 D H$ samples.
	\label{thm:gen-rl}
\end{theorem}

\begin{algorithm*}[h]\caption{Learn policy with query model.}\label{alg:querypoly}
    \begin{algorithmic}[1]
%    \State {\bf Input:} Failure probability $\delta$, precision $\epsilon$. \jnote{Aren't these both 0??} (Jiaqi: True, this is not added by me...)
    %Set $n$ as in Theorem~\ref{thm:retreive_nn1} for $\F_{NN1}$ or Theorem~\ref{thm:retreive_nn2} for $\F_{NN2}$.
    \For{$h=1, \cdots, H$}
        %\State \Comment{$n_1 = \mathrm{Poly}(d,k,\kappa,1/\epsilon,\log(1/\delta))$}
        \State randomly choose a generic subset of state-action pairs $\gP_h \subseteq \gS \times \gA$ with size $\abs{\gP_h} = 2D$
        \State query $s' = T(s, a)$ and reward $r(s, a)$ for $(s, a) \in \gP_h$.
    \EndFor
    \end{algorithmic}
    \end{algorithm*}



%\begin{proof}
%    
%    \jnote{Jiaqi: State the theorem from anonymous, and then refer to the stated theorem. We can give this in the main text}
%We show we can recover optimal policy $\pi^\star$ with these samples. We begin with the final step $\pi^\star_H$. To recover it, note that $Q^\star_{H}(s, a) = r(s, a)$, so we can  use Theorem \ref{thm} in \citep{concurrent} to recover $f_H$. Finally, we can compute $\pi^\star_H(s) = \arg \max_{a \in \gA} Q^\star_H(s, a) = \arg \max_{a \in \gA} f_H(s, a)$. 
%
%Given $\pi^\star_{h+1}, \cdots, \pi^\star_H$, we show how to recover $\pi^\star_H$. First, because we have the optimal policy for steps $h+1$ to $H$, we can compute $V^\star_{h+1}(s)$ for $s \in \gS$. Secondly, for $(s, a) \in \gP_h$, we compute $Q^\star(s, a) = r(s, a) + V^\star_{h+1}(T(s, a))$. At last, we use Theorem \ref{thm} in \citep{concurrent} to recover $f_h$. By induction, we can recover $Q^\star_H, Q^\star_{H-1}, \cdots, Q^\star_1$, and obtain the optimal policy.
%\end{proof}

We give two important examples of admissible polynomial families with low dimension.
\begin{example} (Low-rank Polynomial)
The function  $f\in \mathcal{F}_{\gV}$ is a polynomial with $k$ terms, that is 
	\begin{equation*}
F(x) =  \sum_{i = 1}^k \lambda_i \langle v_i, x \rangle^{p_i}, \label{eq:poly:1}
	\end{equation*}
	where $p  = \max\{p_i\}$. The $\lambda_i v_i$ are unknown parameters. The dimension of this family is upper bounded by $D \le dr$.
	\end{example}
\begin{example}
	
	The function $ f \in \mathcal{F}_\gV$ is of the form $f(x) = q(Ux)$, where $U \in \mathbb{R}^{k \times d}$ and $q$ is a degree $p$ polynomial. The polynomial $q$ and matrix $U$ are unknown parameters. The dimension of this family is upper bounded by $ D \le  d (k+1)^p$.
\end{example}

\subsubsection{Online RL}
In this subsection, we show that under a strong but necessary assumption on the feature map $\phi_h$, a polynomial realizable MDP can be efficiently learned.
\begin{theorem} Assume that $\{\phi_h(s, a) \mid a\in \gA\}$ is generic for every state $s$ at every level $h$. Under polynomial realizability. Then within $T = 2 DH$ episodes, we can almost surely obtain the optimal policy $\pi^\star$. \label{thm4} 
%   \jnote{Define r, defnite assumptioins on Q}
\end{theorem}

\begin{algorithm*}[h]\caption{Learn policy online RL.}\label{alg:onlinerlpoly}
    \begin{algorithmic}[1]
%    \State {\bf Input:} Failure probability $\delta$, precision $\epsilon$. 
    %Set $n$ as in Theorem~\ref{thm:retreive_nn1} for $\F_{NN1}$ or Theorem~\ref{thm:retreive_nn2} for $\F_{NN2}$.
    \For{$h=H,\ldots 1$}
        %\State \Comment{$n_1 = \mathrm{Poly}(d,k,\kappa,1/\epsilon,\log(1/\delta))$}
        \For{$i \in [2D]$}
            \State play random action on step $h' \le h$, and choose $\arg \max_{a} Q^\star(s, a)$ on steps $h' \ge h$
        \EndFor
    \EndFor
    \end{algorithmic}
    \end{algorithm*}


%The proof is essentially the same as that of Theorem \ref{thm3}.

%\begin{proof} We define $\gP_h = \{\phi_h(s_h^k) : (H-h)2dr < k \le (H-h+1)2dr\}$.
%
%We show we can recover optimal policy $\pi^\star$. We begin with the final step $\pi^\star_H$. For every $h \in [H]$, since $\{T_h(s_h, a) \mid a \in \gA\}$ is generic, we have that $\gP_h$ is generic almost surely. The rest of the proof is the same as the proof of Theorem \ref{thm3}.
%\end{proof}

%%%%%% backup for "generic trnsition" %%%%%%% 
% \subsubsection{Online RL}
% In this subsection, we show that under a strong but necessary assumption on the transition dynamics, a polynomial realizable MDP can be efficiently learned.
% \begin{theorem} Assume that $\{T_h(s, \cdot) \mid a\in \gA\}$ is generic for every state $s$ and polynomial realizability. Then within $T = 2 DH$ episodes, we can almost surely obtain the optimal policy $\pi^\star$. \label{thm4} 
% %	\jnote{Define r, defnite assumptioins on Q}
% \end{theorem}

% \begin{algorithm*}[h]\caption{Learn policy online RL.}\label{alg:onlinerlpoly}
%     \begin{algorithmic}[1]
% %    \State {\bf Input:} Failure probability $\delta$, precision $\epsilon$. 
%     %Set $n$ as in Theorem~\ref{thm:retreive_nn1} for $\F_{NN1}$ or Theorem~\ref{thm:retreive_nn2} for $\F_{NN2}$.
%     \For{$h=H,\ldots 1$}
%         %\State \Comment{$n_1 = \mathrm{Poly}(d,k,\kappa,1/\epsilon,\log(1/\delta))$}
%         \For{$i \in [2D]$}
%             \State play random action on step $h' \le h$, and choose $\arg \max_{a} Q^\star(s, a)$ on steps $h' \ge h$
%         \EndFor
%     \EndFor
%     \end{algorithmic}
%     \end{algorithm*}


% %The proof is essentially the same as that of Theorem \ref{thm3}.

% %\begin{proof} We define $\gP_h = \{\phi_h(s_h^k) : (H-h)2dr < k \le (H-h+1)2dr\}$.
% %
% %We show we can recover optimal policy $\pi^\star$. We begin with the final step $\pi^\star_H$. For every $h \in [H]$, since $\{T_h(s_h, a) \mid a \in \gA\}$ is generic, we have that $\gP_h$ is generic almost surely. The rest of the proof is the same as the proof of Theorem \ref{thm3}.
% %\end{proof}

==> sections/poly_backup.tex <==

\subsection{Deterministic Transitions and Generative Model}

%Setting: we obtain $N$ samples from each state-action pair. 
%
%Assumption: for every $h = 1, \cdots, H$, the set $\{\phi_h(s, a) \mid s \in \gS, a \in \gA\}$ is generic.
%\jnote{Jiaqi: State algorithm?} \jnote{All proofs go in supplementary, deadline is 6-4 for proofs.} \jnote{State setting! what's the assumption on Q*????}

\begin{definition}[Admissible Polynomial Family]
Define $\mathcal{X}: = \left\{\begin{bmatrix} 1 \\ x \end{bmatrix}^{\otimes p}: x \in \mathbb{R}^d\right\}$. Define $\F_{\gV}:=\{f_\Theta(x)= \left\langle \Theta, \begin{bmatrix} 1 \\ x \end{bmatrix}^{\otimes p}\right \rangle: \Theta \in \mathcal{V}  \}$ for a variety $\mathcal{V}$ as a polynomial family. $\F_{\gV}$ is said to be admissible\footnote{Admissible means the dimension of $\mathcal{X}$ decreases by one when there is an additional linear constraint $\langle \Theta, X\rangle =0$} wrt $\mathcal{X}$ if for any $\Theta \in \gV$, $\text{dim}(\mathcal{X} \cap \{X \in \mathcal{X} : \langle X,  \Theta\rangle =0\rangle\}  )< \text{dim}(\mathcal{X})=d $. 
%The dimension $D$ of the family is the algebraic dimension of the variety $\mathcal{V}$. 

The dimension $D$ of the family is the dimension of $\gV$.

%We further assume that $\mathcal{V}$ is the finite union of irreducible algebraic varieties\footnote{This can be weakened to containment in the finite union of irreducible varieties.}.

\end{definition}
\begin{theorem}[\cite{Anonymous}]
%	\textcolor{red}{\bf JIAQI Please summarize the bandit theorem here that we invoke}
%	
%	Let $\mathcal{V}$ be the finite union of irreducible algebraic varieties and the Minkowski set difference $\mathcal{V} - \mathcal{V}$ has  dimension $D$. Consider a polynomial family  $p_\Theta(x)= \left\langle \Theta, \begin{bmatrix} 1 \\ x \end{bmatrix}^{\otimes p}\right \rangle$ with coefficients $\Theta \in \mathcal{V}$.
% Then for any $n\ge D$, there is a unique solution (or no solution) $\Theta^\ast$ to the system of equations $y_i = p_\Theta(x_i)$, for almost all $(x_1,\ldots, x_n)$ with respect to the product measure on $\mathbb{R}^{d} \times \cdots \times \mathbb{R}^d$.
Consider the polynomial family $\F_{\gV}$ of dimension $D$.  For $n \ge 2D$, there is a unique solution (or no solution) to the system of equations $y_i =f(x_i)$ for $f \in \F_{\gV}$ almost surely with respect to the product measure on $\mathbb{R}^d \times \ldots \mathbb{R}^d$.



	\end{theorem}
\begin{assumption}[Polynomial Realizability]
For all $ h \in [H]$,  $Q^\ast_h \in \F_{\gV}$ for an admissible polynomial family.
\end{assumption}

%\jnote{What is r???} what's the model class???? ??? 
\begin{theorem} Under the polynomial realizability, Algorithm \ref{alg:querypoly} learns the optimal policy $\pi^\star$ with at most  $N = 2 D H$ samples.
	\label{thm:gen-rl}
\end{theorem}

\begin{algorithm*}[h]\caption{Learn policy with query model.}\label{alg:querypoly}
    \begin{algorithmic}[1]
%    \State {\bf Input:} Failure probability $\delta$, precision $\epsilon$. \jnote{Aren't these both 0??} (Jiaqi: True, this is not added by me...)
    %Set $n$ as in Theorem~\ref{thm:retreive_nn1} for $\F_{NN1}$ or Theorem~\ref{thm:retreive_nn2} for $\F_{NN2}$.
    \For{$h=1, \cdots, H$}
        %\State \Comment{$n_1 = \mathrm{Poly}(d,k,\kappa,1/\epsilon,\log(1/\delta))$}
        \State randomly choose a generic subset of state-action pairs $\gP_h \subseteq \gS \times \gA$ with size $\abs{\gP_h} = 2dr$
        \State query $s' = T(s, a)$ and reward $r(s, a)$ for $(s, a) \in \gP_h$.
    \EndFor
    \end{algorithmic}
    \end{algorithm*}



%\begin{proof}
%    
%    \jnote{Jiaqi: State the theorem from anonymous, and then refer to the stated theorem. We can give this in the main text}
%We show we can recover optimal policy $\pi^\star$ with these samples. We begin with the final step $\pi^\star_H$. To recover it, note that $Q^\star_{H}(s, a) = r(s, a)$, so we can  use Theorem \ref{thm} in \citep{concurrent} to recover $f_H$. Finally, we can compute $\pi^\star_H(s) = \arg \max_{a \in \gA} Q^\star_H(s, a) = \arg \max_{a \in \gA} f_H(s, a)$. 
%
%Given $\pi^\star_{h+1}, \cdots, \pi^\star_H$, we show how to recover $\pi^\star_H$. First, because we have the optimal policy for steps $h+1$ to $H$, we can compute $V^\star_{h+1}(s)$ for $s \in \gS$. Secondly, for $(s, a) \in \gP_h$, we compute $Q^\star(s, a) = r(s, a) + V^\star_{h+1}(T(s, a))$. At last, we use Theorem \ref{thm} in \citep{concurrent} to recover $f_h$. By induction, we can recover $Q^\star_H, Q^\star_{H-1}, \cdots, Q^\star_1$, and obtain the optimal policy.
%\end{proof}

We give two important examples of admissible polynomial families with low dimension.
\begin{example} (Low-rank Polynomial)
The function  $f\in \mathcal{F}_{\gV}$ is a polynomial with $k$ terms, that is 
	\begin{equation*}
F(x) =  \sum_{i = 1}^k \lambda_i \langle v_i, x \rangle^{p_i}, \label{eq:poly:1}
	\end{equation*}
	where $p  = \max\{p_i\}$. The $\lambda_i v_i$ are unknown parameters. The dimension of this family is upper bounded by $D \le 2dr$.
	\end{example}
\begin{example}
	
	The function $ f \in \mathcal{F}_\gV$ is of the form $f(x) = q(Ux)$, where $U \in \mathbb{R}^{k \times d}$ and $q$ is a degree $p$ polynomial. The polynomial $q$ and matrix $U$ are unknown parameters. The dimension of this family is upper bounded by $ D \le 2 d (k+1)^p$.
\end{example}
\subsubsection{Online RL}
In this subsection, we show that under a strong but necessary assumption on the transition dynamics, a polynomial realizable MDP can be efficiently learned.
\begin{theorem} Assume that $\{T_h(s, \cdot) \mid a\in \gA\}$ is generic for every state $s$ and polynomial realizability. Then within $T = 2 DH$ episodes, we can almost surely obtain the optimal policy $\pi^\star$. \label{thm4} 
%	\jnote{Define r, defnite assumptioins on Q}
\end{theorem}

\begin{algorithm*}[h]\caption{Learn policy online RL.}\label{alg:onlinerlpoly}
    \begin{algorithmic}[1]
%    \State {\bf Input:} Failure probability $\delta$, precision $\epsilon$. 
    %Set $n$ as in Theorem~\ref{thm:retreive_nn1} for $\F_{NN1}$ or Theorem~\ref{thm:retreive_nn2} for $\F_{NN2}$.
    \For{$h=H,\ldots 1$}
        %\State \Comment{$n_1 = \mathrm{Poly}(d,k,\kappa,1/\epsilon,\log(1/\delta))$}
        \For{$i \in [2D]$}
            \State play random action on step $h' \le h$, and choose $\arg \max_{a} Q^\star(s, a)$ on steps $h' \ge h$
        \EndFor
    \EndFor
    \end{algorithmic}
    \end{algorithm*}


%The proof is essentially the same as that of Theorem \ref{thm3}.

%\begin{proof} We define $\gP_h = \{\phi_h(s_h^k) : (H-h)2dr < k \le (H-h+1)2dr\}$.
%
%We show we can recover optimal policy $\pi^\star$. We begin with the final step $\pi^\star_H$. For every $h \in [H]$, since $\{T_h(s_h, a) \mid a \in \gA\}$ is generic, we have that $\gP_h$ is generic almost surely. The rest of the proof is the same as the proof of Theorem \ref{thm3}.
%\end{proof}

==> sections/results.tex <==
\section{Neural Net Completeness}

\jnote{temporary sec names}

==> structured_rl_large.tex <==
\def\usebigfont{1}
\input{neurips_rl}
